On the Regret of Online Edge Service Hosting

We consider the problem of service hosting where a service provider can dynamically rent edge resources via short term contracts to ensure better quality of service to its customers. The service can also be partially hosted at the edge, in which case, customers' requests can be partially served at the edge. The total cost incurred by the system is modeled as a combination of the rent cost, the service cost incurred due to latency in serving customers, and the fetch cost incurred as a result of the bandwidth used to fetch the code/databases of the service from the cloud servers to host the service at the edge. In this paper, we compare multiple hosting policies with regret as a metric, defined as the difference in the cost incurred by the policy and the optimal policy over some time horizon $T$. In particular we consider the Retro Renting (RR) and Follow The Perturbed Leader (FTPL) policies proposed in the literature and provide performance guarantees on the regret of these policies. We show that under i.i.d stochastic arrivals, RR policy has linear regret while FTPL policy has constant regret. Next, we propose a variant of FTPL, namely Wait then FTPL (W-FTPL), which also has constant regret while demonstrating much better dependence on the fetch cost. We also show that under adversarial arrivals, RR policy has linear regret while both FTPL and W-FTPL have regret $\mathrm{O}(\sqrt{T})$ which is order-optimal.

==> introduction.tex <==
%\color{magenta}

Software as a Service (SaaS) instances like online navigation platforms, Video-on-Demand services, etc., have stringent latency constraints in order to provide a good quality of experience to their customers. While most SaaSs use cloud resources, low latency necessitates the use of storage/computational resources at the edge, i.e., close to the end-user. A service is said to be hosted at the edge if the code and databases needed to serve user queries are stored on the edge servers and requests can be served at the edge. In this work, the service can also be partially hosted at the edge, in which case,  customers' requests can be partially served at the edge \cite{prakash2020partial, LN_partial_hosting}. \color{blue} For instance, consider a SaaS application which can be used to access news articles on demand. A typical news article includes some text, some images and possibly some embedded videos. One way to partially host such a service is to store the text corresponding to the news articles at the edge and store the images/videos in the cloud. Each user request will then be served partially by the edge. 
%For example consider the news application where there are text, image and video requests, in partial service hosting text request can be served by edge and images, videos can be loaded from cloud. 
\color{black}\footnote{This work is supported by a SERB grant on Leveraging Edge Resources for Service Hosting and a SERB grant on Online Learning with Constraints.} 

We consider the setting where third-party resources can be rented via short-term contracts to host the service, and the edge hosting status of the SaaS can be dynamically changed over time. If the service is not hosted at the edge, it can be fetched from the cloud servers  by incurring a fetch cost. The performance of a hosting policy is a function of the rent cost, the fetch cost, and the quality of experience of the users.  We refer to the algorithmic challenge of determining what fraction of the service to host at the edge over time as the \emph{service hosting problem}. \color{blue}Note that we study the service hosting problem from the perspective of a specific SaaS provider in the setting where third-party edge resources can be rented by the provider to improve their cumtomers' quality of experience by reducing latency.  
%The presence of other SaaS providers in the system is captured through the cost of renting resources
%we are considering the problem in application provider perspective and the edge resources are rented by the third-party. So hosting other applications at edge is not a constraint for the service provider but for the third party resource provider. Therefore we consider that resources are always available for service provider and rent cost is known.
\color{black}


%\begin{comment}
Novel online service hosting policies with provable performance guarantees have been proposed in \cite{narayana2021renting, zhao2018red}.
%Online hosting policies make hosting decisions without the knowledge of the future arrival sequence. A commonly used benchmark to compare the performance of such online policies is the offline optimal policy which knows the entire request arrival sequence apriori and uses this information to make hosting decisions.
The metric of interest in \cite{narayana2021renting,zhao2018red} is the \emph{competitive ratio}, defined as the ratio of the cost incurred by an online policy to the cost incurred by an offline optimal policy for the same request arrival sequence. Since the competitive ratio is multiplicative by definition, the absolute value of the difference in the cost incurred by an online policy and the optimal policy can be large even though the competitive ratio of the online policy is close to one. This motivates studying the performance of candidate policies in terms of \emph{regret}, defined as the difference in the cost incurred by the policy and the optimal policy. Regret is a widely used metric in online learning \cite{lai1985asymptotically}, including recently for the caching problem \cite{paschos2019learning,bhattacharjee2020fundamental} which is closely related to the service hosting problem. In this work, one of our goals is to design hosting policies with provable guarantees in terms of the regret. Another key dimension in the performance guarantees of online policies is the assumption made on the request arrival process. Commonly studied settings include the \emph{stochastic setting} and the \emph{adversarial setting}, and
%In the stochastic setting, the arrival process is modeled as a stochastic process whose distribution is not known to the online algorithm. In the adversarial setting, no structural assumptions are made on the arrival process and worst-case guarantees are provided.
 we provide performance guarantees for both settings.

For the service hosting problem, \cite{LN_partial_hosting} proposed the Retro-Renting (RR) policy and showed that it has a constant competitive ratio with respect to the offline optimal policy \color{blue} for only one level of partial hosting of service\color{black}. On the other hand, for the closely related caching problem, several policies inspired by the recent advances in online convex optimization have been proposed including Online Gradient Ascent \cite{paschos2019learning}, Online Mirror Descent \cite{salem2021no}, and Follow the Perturbed Leader (FTPL) \cite{mukhopadhyay2021online,bhattacharjee2020fundamental}. In particular, FTPL has been shown to have order-optimal regret for the caching problem in the adversarial setting  \cite{mukhopadhyay2021online,bhattacharjee2020fundamental}.  In this work, we study regret for the RR and FTPL policies for the service hosting problem, under both the stochastic and adversarial settings. 
Since RR is a deterministic policy, its regret performance in the adversarial setting is poor. On the other hand, a limitation of FTPL is that it makes hosting decisions {agnostic of the fetch cost}. As a result, in some cases, FTPL is prone to fetching and evicting the service multiple times in the initial time-slots when its estimate of the request arrival rate is noisy, thus leading to poor performance.
%\end{comment}

\subsection{Our Contributions}
We propose a variant of the FTPL policy called Wait then Follow the Perturbed Leader (W-FTPL). W-FTPL is a randomized policy that {takes into account the fetch cost in its decision-making}. More specifically, W-FTPL does not fetch the service for an initial wait period which depends on the request arrivals and is an increasing function of the fetch cost. Following the wait period, W-FTPL mimics the FTPL policy.

For i.i.d. stochastic request arrivals and the regret metric, we show that RR is sub-optimal while FTPL and W-FTPL are both order-optimal with respect to the time horizon. While the regret of FTPL can increase linearly with the fetch cost, the regret of W-FTPL increases at most poly logarithmically. The improved performance of W-FTPL over FTPL is a consequence of the fact that W-FTPL avoids most of the fetches made by FTPL in the initial time-slots and by the end of the wait period, its estimate of the arrival rate is accurate enough to avoid multiple fetches. 
%W-FTPL and FTPL also outperform RR in terms of the competitive ratio.
%Further, W-FTLP also outperforms FTLP and RR in simulations.

For the adversarial setting, we first characterize a fundamental lower bound on the regret of any online hosting policy. In terms of regret, we then show that RR is strictly suboptimal, while FTPL and W-FTPL have order-optimal performance with respect to time. 
%For the adversarial setting, the competitive ratio of FTPL and W-FTPL can increase with the fetch cost while that of RR decreases with fetch cost. 

%In recent times there is increase in computational demand for mobile users because of many applications using complex learning algorithms to enhance the user experience. One way to reduce the computational demand from mobile user is to use cloud computing and provide Software as a service (SaaS). In this the user requests a query and computations are done at the back-end servers to provide the result back to the user. The issue with the cloud computing is the latency (few ms). There are many applications which are not tolerant with this latency and need much faster response to run the application smoothly. Edge computing is considered as one of the solution to deal with latency. In the edge computing apart from back-end server (cloud server) which has huge computational power it also has a front-end server (edge server) close to the user but has limited computational power compared to back-end server. Any request from the user first comes to the edge server and if the edge server was unable to serve the request due to the load on it or for any other reason then the request will be forwarded to the cloud where the computations are done and the result is forwarded to the user. Since the edge server is closer to users the latency incurred is  much less than in cloud computing.

%We consider a system where the edge servers are rented from resource providers like Amazon, Google, etc., to host the service. There is a cost for forwarding the request to back-end server if it was not served at the edge. Apart from that we consider the cost of fetching a service from back-end to edge server called as \emph{fetch cost}. Since the edge servers are rented for a fixed duration and can change the renting status only after that duration, we consider a time slotted system. We can either host the service or not host the service in each time slot which is decided by the policy we consider. The request arrivals at the edge may or may not follow any distribution, so we need an on-line policy which performs well for any type of request sequence. Another way to look at it is that the policy should perform well for both stochastic and adversarial arrivals.

%To compare different policies and to decide which policy performs better we need some metrics of comparison. The metrics we considered are expected regret and competitive ratio which are widely used in literature to evaluate on-line policies.  The regret is defined as the difference between the cost of the policy  considered and the optimal static policy (see section \ref{sec:setting} for more details about regret). Smaller the regret better the policy. Competitive ratio is defined as the ratio between the expected cost of the policy and the cost of optimal policy (see section \ref{sec:setting} for more details about competitive ratio). Smaller the competitive ratio better the policy.

%Retro Renting (RR) policy in \cite{narayana2021renting} is one of the on-line policies which fits exactly to the model we considered. It is a deterministic policy which considers both fetch cost and rent cost along with past arrivals till the previous fetch or evict has happened for making decisions. This policy is analyzed by considering competitive ratio as a metric in \cite{narayana2021renting} and shown that as fetch cost increases competitive ratio decreases. Since it is a deterministic policy this policy inccurs high regret in case of adversarial arrivals.
%Follow The Perturbed Leader (FTPL)  is another on-line policy  which is there in file caching literature and we mapped it to our setting. It is a randomized policy and considers rent cost along with all the requests seen till that point for making decisions and ignores the fetch cost. Since FTPL ignores fetch cost the regret of FTPL policy can be high for large fetch cost due to multiple fetches. The FTPL policy performs well in case of stochastic and adversarial arrivals for small fetch cost. As the fetch cost increases the performance degrades. So we need a policy which performs good in terms of regret for large fetch cost and for stochastic, adversarial arrival processes. 



==> relatedWork.tex <==
In this section we discuss already existing literature related to our work. Novel online service hosting policies with provable performance guarantees have been proposed in \cite{narayana2021renting, zhao2018red}. \cite{fan2022online} considers service hosting along with service routing, where service hosting decides whether to host the service at edge or not and service routing decides when to route the request to cloud server.
%Online hosting policies make hosting decisions without the knowledge of the future arrival sequence. A commonly used benchmark to compare the performance of such online policies is the offline optimal policy which knows the entire request arrival sequence apriori and uses this information to make hosting decisions.
The metric of interest in \cite{narayana2021renting,zhao2018red} is the \emph{competitive ratio}, defined as the ratio of the cost incurred by an online policy to the cost incurred by an offline optimal policy for the same request arrival sequence. Since the competitive ratio is multiplicative by definition, the absolute value of the difference in the cost incurred by an online policy and the optimal policy can be large even though the competitive ratio of the online policy is close to one. This motivates studying the performance of candidate policies in terms of \emph{regret}, defined as the difference in the cost incurred by the policy and the offline optimal policy. Regret is a widely used metric in online learning \cite{lai1985asymptotically}, including recently for the caching problem \cite{paschos2019learning,bhattacharjee2020fundamental,bura2021learning} which is closely related to the service hosting problem. In this work, one of our goals is to design hosting policies with provable guarantees in terms the regret. Another key dimension in the performance guarantees of online policies is the assumption made on the request arrival process. Commonly studied settings include the \emph{stochastic setting} and the \emph{adversarial setting} and
%In the stochastic setting, the arrival process is modeled as a stochastic process whose distribution is not known to the online algorithm. In the adversarial setting, no structural assumptions are made on the arrival process and worst-case guarantees are provided.
we provide performance guarantees for both settings.

For the service hosting problem, \cite{narayana2021renting} proposed the Retro-Renting (RR) policy and showed that it has a constant competitive ratio with the offline optimal policy. On the other hand, for the closely related caching problem, several policies inspired by the recent advances in online convex optimization have been proposed including Online Gradient Ascent \cite{paschos2019learning}, Online Mirror Descent \cite{salem2021no} and Follow the Perturbed Leader (FTPL) \cite{mukhopadhyay2021online,bhattacharjee2020fundamental}. In particular, FTPL has been shown to have order-optimal regret for the caching problem in the adversarial setting  \cite{mukhopadhyay2021online,bhattacharjee2020fundamental}.  Similarly one can use the polices in online convex optimization in service caching problem setup as well. Apart from FTPL policy there are policies like exponential weighted algorithm (Hedge) \cite{mourtada2019optimality}, Follow Lazy Leader (FLL) \cite{kalai2005efficient} in online convex optimization literature which also provide order-optimal regret in adversarial setting. Since these algorithms are designed for adversarial arrivals it is not clear if the same algorithm is optimal in stochastic setting as well. In \cite{mourtada2019optimality} it is shown that Hedge is optimal in both stochastic and adversarial setting \emph{without any switching cost}. So it is not clear whether Hedge policy is optimal or not if there is switching cost.
In this work, we study regret for the RR and FTPL policies for the service hosting problem, under both the stochastic and adversarial settings. Since RR is a deterministic policy, its regret performance in the adversarial setting is poor. A limitation of FTPL which is a randomized policy is that it makes hosting decisions agnostic of the fetch cost. As a result, in some cases, FTPL is prone to fetching and evicting the service multiple times in the initial time-slots when its estimate of the request arrival rate is noisy, thus leading to poor performance.



